Tau Be or not Tau Be? - A Perspective on Service Compatibility and Substitutability

One of the main open research issues in Service Oriented Computing is to propose automated techniques to analyse service interfaces. A first problem, called compatibility, aims at determining whether a set of services (two in this paper) can be composed together and interact with each other as expected. Another related problem is to check the substitutability of one service with another. These problems are especially difficult when behavioural descriptions (i.e., message calls and their ordering) are taken into account in service interfaces. Interfaces should capture as faithfully as possible the service behaviour to make their automated analysis possible while not exhibiting implementation details. In this position paper, we choose Labelled Transition Systems to specify the behavioural part of service interfaces. In particular, we show that internal behaviours (tau transitions) are necessary in these transition systems in order to detect subtle errors that may occur when composing a set of services together. We also show that tau transitions should be handled differently in the compatibility and substitutability problem: the former problem requires to check if the compatibility is preserved every time a tau transition is traversed in one interface, whereas the latter requires a precise analysis of tau branchings in order to make the substitution preserve the properties (e.g., a compatibility notion) which were ensured before replacement.

==> eptcsdata.tex <==
\providecommand{\firstpage}{57}
\providecommand{\publicationstatus}{C\'amara, Canal, and Sala\"un (Eds.) \\
Component and Service Interoperability (WCSI10)\\
EPTCS 37, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.37.5}{10.4204/EPTCS.37.5}}

